AdaCoder: An Adaptive Planning and Multi-Agent Framework for Function-Level Code Generation

Recently, researchers have proposed many multi-agent frameworks for function-level code generation, which aim to improve software development productivity by automatically generating function-level source code based on task descriptions. A typical multi-agent framework consists of Large Language Model (LLM)-based agents that are responsible for task planning, code generation, testing, debugging, etc. Studies have shown that existing multi-agent code generation frameworks perform well on ChatGPT. However, their generalizability across other foundation LLMs remains unexplored systematically. In this paper, we report an empirical study on the generalizability of four state-of-the-art multi-agent code generation frameworks across six open-source LLMs with varying parameter sizes, architectures, and performance levels. Our study reveals the unstable generalizability of existing frameworks on diverse foundation LLMs. Based on the findings obtained from the empirical study, we propose AdaCoder, a novel adaptive planning, multi-agent framework for function-level code generation. AdaCoder has two phases. Phase-1 is an initial code generation step without planning, which uses an LLM-based coding agent and a script-based testing agent to unleash LLM's native power, identify cases beyond LLM's power, and determine the errors hindering execution. Phase-2 adds a rule-based debugging agent and an LLM-based planning agent for iterative code generation with planning. Our evaluation shows that AdaCoder achieves higher generalizability on diverse LLMs. Compared to the best baseline MapCoder, AdaCoder is on average 27.69% higher in Pass@1, 16 times faster in inference, and 12 times lower in token consumption.

==> discussion.tex <==
\subsection{Ablation Study}

\begin{table*}
    \scriptsize
    \centering
    \caption{Ablation study results of AdaCoder with different agents removed, applied to six open-source models and four closed-source models. "w/o Prompt" indicates the removal of the Prompt Engineer, while "w/o Debug" indicates the removal of the Debug Specialist.} 
    \begin{tabular}{lcccc}
        \toprule
        \textbf{LLMs} & \textbf{AdaCoder} & \textbf{w/o Prompt} & \textbf{w/o Debug} & \textbf{w/o Prompt \& Debug} \\
        \midrule
        CodeLlama-Python-7B & 63.41 & 48.78 (\textcolor{red}{$\downarrow$23.07\%}) & 58.54 (\textcolor{red}{$\downarrow$07.68\%}) & 41.46 (\textcolor{red}{$\downarrow$34.62\%}) \\
        CodeLlama-Python-13B  & 71.95 & 56.71 (\textcolor{red}{$\downarrow$21.18\%}) & 64.63 (\textcolor{red}{$\downarrow$10.17\%}) & 53.66 (\textcolor{red}{$\downarrow$25.42\%}) \\
        CodeLlama-Python-34B & 81.10 & 64.63 (\textcolor{red}{$\downarrow$20.31\%}) & 71.95 (\textcolor{red}{$\downarrow$11.28\%}) & 57.93 (\textcolor{red}{$\downarrow$28.57\%}) \\
        DeepSeek-Coder-1.3B & 76.83 & 62.20 (\textcolor{red}{$\downarrow$19.04\%}) & 70.12 (\textcolor{red}{$\downarrow$08.73\%}) & 54.27 (\textcolor{red}{$\downarrow$29.36\%}) \\
        DeepSeek-Coder-6.7B & 85.98 & 72.56 (\textcolor{red}{$\downarrow$15.61\%}) & 79.27 (\textcolor{red}{$\downarrow$07.80\%}) & 57.93 (\textcolor{red}{$\downarrow$32.62\%}) \\
        DeepSeek-Coder-33B & 90.85 & 74.39 (\textcolor{red}{$\downarrow$18.12\%}) & 70.73 (\textcolor{red}{$\downarrow$22.15\%}) & 61.59 (\textcolor{red}{$\downarrow$32.21\%}) \\
        GPT-3.5-turbo & 96.95 & 75.61 (\textcolor{red}{$\downarrow$22.01\%}) & 86.59 (\textcolor{red}{$\downarrow$10.69\%}) & 76.22 (\textcolor{red}{$\downarrow$21.38\%}) \\
        GPT-4 & 96.95 & 81.71 (\textcolor{red}{$\downarrow$15.72\%}) & 90.24 (\textcolor{red}{$\downarrow$06.92\%}) & 79.27 (\textcolor{red}{$\downarrow$18.24\%}) \\
        GPT-4-turbo & 98.17 & 91.46 (\textcolor{red}{$\downarrow$06.84\%}) & 92.07 (\textcolor{red}{$\downarrow$06.21\%}) & 90.24 (\textcolor{red}{$\downarrow$08.08\%}) \\
        GPT-4o & 98.17 & 91.46 (\textcolor{red}{$\downarrow$06.84\%}) & 93.90 (\textcolor{red}{$\downarrow$04.35\%}) & 89.02 (\textcolor{red}{$\downarrow$09.32\%}) \\
        \midrule
        $\Delta$ Average & - & \textcolor{red}{$\downarrow$16.87\%} & \textcolor{red}{$\downarrow$09.60\%} & \textcolor{red}{$\downarrow$23.98\%} \\
        \bottomrule
    \end{tabular}
\label{tab_ablation}
\end{table*}

As described in Section \ref{method}, among AdaCoder's four agents, the Programming Assistant and Code Evaluator form the core components and cannot be removed. In contrast, the Prompt Engineer and Debug Specialist are auxiliary agents designed to enhance code generation capabilities and can be removed in ablation experiments. Consequently, we selected six open-source LLMs from RQ1 and four closed-source LLMs from RQ3, totaling ten LLMs as foundation models, to evaluate AdaCoder's pass@1 under three conditions on the HumanEval datasets: removing the Prompt Engineer, removing the Debug Specialist, and removing both the Prompt Engineer and Debug Specialist. 
% The experimental results are presented in Table \ref{tab_ablation}.

Table \ref{tab_ablation} shows that in all three scenarios, compared to the complete AdaCoder, the code generation capabilities of all LLMs decreased to varying degrees. Specifically, removing the Prompt Engineer resulted in a decrease in code generation capability ranging from 6.84\% to 23.07\% across the LLMs, with an average decrease of 16.87\%. CodeLlama-Python-7B experienced the largest decrease, while GPT-4-turbo and GPT-4o showed the smallest decrease. This phenomenon may be attributed to the latter two's inherently strong code generation capabilities, rendering the strategies designed by the Prompt Engineer less impactful. Removing the Debug Specialist led to a decrease in code generation capability ranging from 4.35\% to 22.15\%, with an average decrease of 9.60\%. DeepSeek-Coder-33B exhibited the largest decrease, while GPT-4o showed the smallest. This disparity might be due to GPT-4o being less prone to generating simple errors. Simultaneously removing both the Prompt Engineer and Debug Specialist resulted in a decrease in code generation capability ranging from 8.08\% to 34.62\%, with an average decrease of 23.98\%. CodeLlama-Python-7B experienced the largest decrease, while GPT-4-turbo showed the smallest. These results demonstrate the contributions of each component in AdaCoder.

% \vspace{0.3cm}
% \begin{mdframed}[nobreak=true]
% \textbf{Answer:} In AdaCoder, the Programming Assistant and Code Evaluator are essential core components. The Prompt Engineer and Debug Specialist enhance code generation performance: Removing the Prompt Engineer decreases code generation capability by 16.87\%, the Debug Specialist by 9.60\%, and both by 23.98\%.
% \end{mdframed}

\subsection{Limitations and Threats to Validity}

We set the iteration count to five by default for AdaCoder's performance and demonstrate how the count can be adjusted to proportionally gain performance at the expense of time and token consumption in Figure \ref{fig_AdaCoder_t_value}. However, for other foundation LLMs and code generation tasks, this parameter may require some adjustment to achieve an optimal balance between pass@1 and resource consumption. Moreover, although our experiments are designed to mirror real-world scenarios, the specific datasets and foundation LLMs employed may restrict the broader applicability of our findings. To mitigate this, we plan to validate our approach using more diverse datasets and in various environments in future research.

% Currently, there is a notable lack of code generation benchmarks and evaluation metrics that accurately reflect real-world software development scenarios. Consequently, our study relied solely on HumanEval and MBPP as code generation evaluation benchmarks, which inevitably introduces some discrepancies compared to actual software development contexts. Nevertheless, AdaCoder's modular design partially mitigates this limitation. Specifically, the Debug Specialist component can be utilized independently as a tool for addressing simple code issues, thereby offering some practical applicability beyond the constraints of the benchmark. Additionally, we set the iteration count to \( t=5 \) for AdaCoder's performance and demonstrate how \( t \) can be adjusted to proportionally gain performance at the expense of time and token consumption in Figure \ref{fig_AdaCoder_t_value}. However, for other foundation models and code generation tasks, this parameter may require some adjustment to achieve an optimal balance between accuracy and resource consumption.

% \textbf{Parameter Optimization.} In this study, we developed AdaCoder, a multi-agent framework comprising four intelligent agents, designed to enhance the code generation capabilities of both open-source and closed-source LLMs. Throughout our experiments, we consistently set the iteration count $t$ of the workflow to 5. However, it is important to note that this parameter may require adjustment for future foundation models and diverse code generation tasks to achieve an optimal balance between accuracy performance and resource consumption.

\subsection{Ablation Study}

\begin{table*}
    \scriptsize
    \centering
    \caption{Ablation study results of AdaCoder with different agents removed, applied to six open-source models and four closed-source models. "w/o Prompt" indicates the removal of the Prompt Engineer, while "w/o Debug" indicates the removal of the Debug Specialist.} 
    \begin{tabular}{lcccc}
        \toprule
        \textbf{LLMs} & \textbf{AdaCoder} & \textbf{w/o Prompt} & \textbf{w/o Debug} & \textbf{w/o Prompt \& Debug} \\
        \midrule
        CodeLlama-Python-7B & 63.41 & 48.78 (\textcolor{red}{$\downarrow$23.07\%}) & 58.54 (\textcolor{red}{$\downarrow$07.68\%}) & 41.46 (\textcolor{red}{$\downarrow$34.62\%}) \\
        CodeLlama-Python-13B  & 71.95 & 56.71 (\textcolor{red}{$\downarrow$21.18\%}) & 64.63 (\textcolor{red}{$\downarrow$10.17\%}) & 53.66 (\textcolor{red}{$\downarrow$25.42\%}) \\
        CodeLlama-Python-34B & 81.10 & 64.63 (\textcolor{red}{$\downarrow$20.31\%}) & 71.95 (\textcolor{red}{$\downarrow$11.28\%}) & 57.93 (\textcolor{red}{$\downarrow$28.57\%}) \\
        DeepSeek-Coder-1.3B & 76.83 & 62.20 (\textcolor{red}{$\downarrow$19.04\%}) & 70.12 (\textcolor{red}{$\downarrow$08.73\%}) & 54.27 (\textcolor{red}{$\downarrow$29.36\%}) \\
        DeepSeek-Coder-6.7B & 85.98 & 72.56 (\textcolor{red}{$\downarrow$15.61\%}) & 79.27 (\textcolor{red}{$\downarrow$07.80\%}) & 57.93 (\textcolor{red}{$\downarrow$32.62\%}) \\
        DeepSeek-Coder-33B & 90.85 & 74.39 (\textcolor{red}{$\downarrow$18.12\%}) & 70.73 (\textcolor{red}{$\downarrow$22.15\%}) & 61.59 (\textcolor{red}{$\downarrow$32.21\%}) \\
        GPT-3.5-turbo & 96.95 & 75.61 (\textcolor{red}{$\downarrow$22.01\%}) & 86.59 (\textcolor{red}{$\downarrow$10.69\%}) & 76.22 (\textcolor{red}{$\downarrow$21.38\%}) \\
        GPT-4 & 96.95 & 81.71 (\textcolor{red}{$\downarrow$15.72\%}) & 90.24 (\textcolor{red}{$\downarrow$06.92\%}) & 79.27 (\textcolor{red}{$\downarrow$18.24\%}) \\
        GPT-4-turbo & 98.17 & 91.46 (\textcolor{red}{$\downarrow$06.84\%}) & 92.07 (\textcolor{red}{$\downarrow$06.21\%}) & 90.24 (\textcolor{red}{$\downarrow$08.08\%}) \\
        GPT-4o & 98.17 & 91.46 (\textcolor{red}{$\downarrow$06.84\%}) & 93.90 (\textcolor{red}{$\downarrow$04.35\%}) & 89.02 (\textcolor{red}{$\downarrow$09.32\%}) \\
        \midrule
        $\Delta$ Average & - & \textcolor{red}{$\downarrow$16.87\%} & \textcolor{red}{$\downarrow$09.60\%} & \textcolor{red}{$\downarrow$23.98\%} \\
        \bottomrule
    \end{tabular}
\label{tab_ablation}
\end{table*}

As described in Section \ref{method}, among AdaCoder's four agents, the Programming Assistant and Code Evaluator form the core components and cannot be removed. In contrast, the Prompt Engineer and Debug Specialist are auxiliary agents designed to enhance code generation capabilities and can be removed in ablation experiments. Consequently, we selected six open-source LLMs from RQ1 and four closed-source LLMs from RQ3, totaling ten LLMs as foundation models, to evaluate AdaCoder's pass@1 under three conditions on the HumanEval datasets: removing the Prompt Engineer, removing the Debug Specialist, and removing both the Prompt Engineer and Debug Specialist. 
% The experimental results are presented in Table \ref{tab_ablation}.

Table \ref{tab_ablation} shows that in all three scenarios, compared to the complete AdaCoder, the code generation capabilities of all LLMs decreased to varying degrees. Specifically, removing the Prompt Engineer resulted in a decrease in code generation capability ranging from 6.84\% to 23.07\% across the LLMs, with an average decrease of 16.87\%. CodeLlama-Python-7B experienced the largest decrease, while GPT-4-turbo and GPT-4o showed the smallest decrease. This phenomenon may be attributed to the latter two's inherently strong code generation capabilities, rendering the strategies designed by the Prompt Engineer less impactful. Removing the Debug Specialist led to a decrease in code generation capability ranging from 4.35\% to 22.15\%, with an average decrease of 9.60\%. DeepSeek-Coder-33B exhibited the largest decrease, while GPT-4o showed the smallest. This disparity might be due to GPT-4o being less prone to generating simple errors. Simultaneously removing both the Prompt Engineer and Debug Specialist resulted in a decrease in code generation capability ranging from 8.08\% to 34.62\%, with an average decrease of 23.98\%. CodeLlama-Python-7B experienced the largest decrease, while GPT-4-turbo showed the smallest. These results demonstrate the contributions of each component in AdaCoder.

% \vspace{0.3cm}
% \begin{mdframed}[nobreak=true]
% \textbf{Answer:} In AdaCoder, the Programming Assistant and Code Evaluator are essential core components. The Prompt Engineer and Debug Specialist enhance code generation performance: Removing the Prompt Engineer decreases code generation capability by 16.87\%, the Debug Specialist by 9.60\%, and both by 23.98\%.
% \end{mdframed}

\subsection{Limitations and Threats to Validity}

We set the iteration count to five by default for AdaCoder's performance and demonstrate how the count can be adjusted to proportionally gain performance at the expense of time and token consumption in Figure \ref{fig_AdaCoder_t_value}. However, for other foundation LLMs and code generation tasks, this parameter may require some adjustment to achieve an optimal balance between pass@1 and resource consumption. Moreover, although our experiments are designed to mirror real-world scenarios, the specific datasets and foundation LLMs employed may restrict the broader applicability of our findings. To mitigate this, we plan to validate our approach using more diverse datasets and in various environments in future research.

% Currently, there is a notable lack of code generation benchmarks and evaluation metrics that accurately reflect real-world software development scenarios. Consequently, our study relied solely on HumanEval and MBPP as code generation evaluation benchmarks, which inevitably introduces some discrepancies compared to actual software development contexts. Nevertheless, AdaCoder's modular design partially mitigates this limitation. Specifically, the Debug Specialist component can be utilized independently as a tool for addressing simple code issues, thereby offering some practical applicability beyond the constraints of the benchmark. Additionally, we set the iteration count to \( t=5 \) for AdaCoder's performance and demonstrate how \( t \) can be adjusted to proportionally gain performance at the expense of time and token consumption in Figure \ref{fig_AdaCoder_t_value}. However, for other foundation models and code generation tasks, this parameter may require some adjustment to achieve an optimal balance between accuracy and resource consumption.

% \textbf{Parameter Optimization.} In this study, we developed AdaCoder, a multi-agent framework comprising four intelligent agents, designed to enhance the code generation capabilities of both open-source and closed-source LLMs. Throughout our experiments, we consistently set the iteration count $t$ of the workflow to 5. However, it is important to note that this parameter may require adjustment for future foundation models and diverse code generation tasks to achieve an optimal balance between accuracy performance and resource consumption.

==> rq3.tex <==





% it is activated when the initially generated code fails to pass tests even after debugging by the Debug Specialist. The Prompt Engineer then designs an implementation strategy based on the problem description to assist the Programming Assistant in code generation. This approach allows the LLM to attempt solutions without initial constraints, providing guidance only after the LLM's independent attempt fails. Furthermore, we add "Let's explore various approaches and perspectives to solve this problem" as a part of prompt to promote Prompt Engineer to generate more diverse strategies. Combining the above operations, we hope this design will encourage the LLM to generate more diverse solutions, following the conclusion from subsection \ref{mapcoder} that promoting diverse solution generation by LLMs and then selecting the optimal one improves the quality of the final result. The Prompt Engineer is solely responsible for designing strategies to assist the Programming Assistant in code generation, and repeat $t$ times. Without the Prompt Engineer, AdaCoder can still function, but we anticipate some degree of performance loss. The detailed prompt received by the Prompt Engineer is shown in Figure \ref{fig_AdaCoder_prompt}. 

% \subsubsection{Innovations in AdaCoder}

% AdaCoder differs from existing multi-agent frameworks in three key aspects: 

% \begin{itemize}
%     \item [$\bullet$] AdaCoder does not use the LLM itself to debug problematic code (a method commonly adopted by the four multi-agent frameworks selected in this study). Instead, it employs rule-based debugging methods that do not consume GPU resources or time. This design is based on the findings in subsection \ref{iteration_refinement}, which indicate that using open-source models for iterative refinement is ineffective and resource-intensive. 
%     \item [$\bullet$] Unlike existing multi-agent frameworks such as AgentCoder, MapCoder and Self-Collaboration, AdaCoder does not preset a code completion strategy for the Programming Assistant in the initial phase. Instead, it provides only the problem description at first, allowing the LLM to independently choose problem-solving approaches. Only when the generated code snippets fail to pass the test after debugged by Debug Specialist, the Prompt Engineer devises a plan to assist Programming Assistant. This design of selective assistance achieves a balance of accuracy and resource consumption. This design idea partly adheres to the conclusion drawn in subsection \ref{mapcoder}, which suggests that encouraging LLMs to generate diverse solutions and then selecting the optimal one enhances the quality of the final result. 
%     \item [$\bullet$] AdaCoder avoids prompt engineering methods like CoT or Few-Shot that significantly increase prompt length and complexity (as used in AgentCoder). Instead, it uses only problem description or Plan + problem description to construct prompts. This design stems from the conclusion in subsection \ref{prompt} that long and structurally complex prompts perform poorly with open-source models. 
% \end{itemize}

% \subsection{Research Questions}

% So far, we have developed an innovative multi-agent framework: AdaCoder. However, its advantages in terms of accuracy, GPU and time resource compared to existing multi-agent frameworks remain to be verified. Therefore, in this evaluation section, we will conduct a systematic experimental analysis centered around the following four research questions: 

% \textbf{RQ3: How does AdaCoder perform on open-source models?} This RQ apply AdaCoder to the six open-source LLMs selected in RQ1 and evaluate its accuracy on the HumanEval dataset. Furthermore, we will investigate the impact of varying the value of max iterations $t$ in algorithm \ref{algo_workflow} on AdaCoder's performance to comprehensively assess its performance in open-source environments.

% \textbf{RQ4: How does AdaCoder perform on closed-source models?} This RQ aim to explore whether AdaCoder can achieve equally excellent results on current SOTA closed-source models, such as the GPT series. Specifically, we will deploy AdaCoder on four closed-source models—GPT-3.5-turbo, GPT-4, GPT-4-turbo, and GPT-4o—and evaluate its accuracy on the HumanEval dataset. These results will be compared with the four multi-agent frameworks selected in RQ1. Similarly, we will analyze the impact of different $t$ values on AdaCoder's performance across closed-source models to assess its adaptability in diverse environments.

% \textbf{RQ5: How do different Agents contribute in AdaCoder?} This RQ aims to quantify the contributions of each Agent within AdaCoder and identify potentially redundant components in the framework by an ablation experiment. Through this analysis, we can gain deeper insights into AdaCoder's internal mechanisms, providing a foundation for future optimizations.

% \textbf{RQ6: What is the resource consumption of AdaCoder?} While AdaCoder may significantly enhance LLM performance, its practicality would be questionable if its resource consumption exceeds that of existing resource-intensive frameworks like MapCoder. Therefore, this RQ aims to meticulously record and analyze AdaCoder's token consumption and inference time on both open-source and closed-source models. These data will be compared with other multi-agent frameworks to comprehensively evaluate AdaCoder's resource efficiency and practical application potential.

% \textbf{RQ7: How does AdaCoder perform on the other dataset?} This RQ aims to investigate AdaCoder's performance on a dataset other than HumanEval. Specifically, we selected the MBPP (Mostly Basic Python Programming) dataset and applied four multi-agent frameworks and AdaCoder to six open-source models and four closed-source models under the same experimental conditions. We tested their code generation accuracy, the number of tokens consumed during inference, and the inference time.


% \subsection{Performance on HumanEval Dataset}
\subsection{Pass@1 Performance}\label{eva_accuracy}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{image/mbpp_sample.pdf}
%     \caption{A schematic diagram of the first sample in MBPP test sets.}
%     \label{fig_mbpp_sample}
% \end{figure}


\subsubsection{Experimental Results}

\begin{table*}
    \footnotesize
    \centering
    \caption{The pass@1 performance of AdaCoder compared to the baseline when applied to six open-source models and four closed-source models.}     
    \begin{tabular}{l|c|c|c|c}
        \toprule
        \multirow{2}{*}{\textbf{LLMs}} & \multicolumn{2}{c|}{\textbf{Baseline}} & \multicolumn{2}{|c}{\textbf{AdaCoder}} \\ 
        \cmidrule{2-5} & HumanEval & MBPP & HumanEval & MBPP \\
        \midrule
        CodeLlama-Python-7B  & 32.69 & 42.12 & 63.41 (\textcolor{red}{$\uparrow$93.97\%}) & 68.40 (\textcolor{red}{$\uparrow$62.39\%}) \\
        CodeLlama-Python-13B & 36.65 & 46.86 & 71.95 (\textcolor{red}{$\uparrow$96.32\%}) & 70.40 (\textcolor{red}{$\uparrow$50.23\%}) \\
        CodeLlama-Python-34B & 43.72 & 49.82 & 81.10 (\textcolor{red}{$\uparrow$85.50\%}) & 76.40 (\textcolor{red}{$\uparrow$53.35\%}) \\
        DeepSeek-Coder-1.3B  & 49.39 & 47.80 & 76.83 (\textcolor{red}{$\uparrow$55.56\%}) & 71.80 (\textcolor{red}{$\uparrow$50.21\%}) \\
        DeepSeek-Coder-6.7B  & 58.54 & 58.60 & 85.98 (\textcolor{red}{$\uparrow$46.87\%}) & 78.00 (\textcolor{red}{$\uparrow$33.11\%}) \\
        DeepSeek-Coder-33B   & 64.63 & 66.40 & 90.85 (\textcolor{red}{$\uparrow$40.57\%}) & 81.40 (\textcolor{red}{$\uparrow$22.59\%}) \\
        GPT-3.5-turbo        & 60.30 & 52.20 & 96.95 (\textcolor{red}{$\uparrow$60.78\%}) & 89.40 (\textcolor{red}{$\uparrow$71.26\%}) \\
        GPT-4                & 67.00 & 68.30 & 96.95 (\textcolor{red}{$\uparrow$44.70\%}) & 90.40 (\textcolor{red}{$\uparrow$32.36\%}) \\
        GPT-4-turbo          & 87.10 & 63.40 & 98.17 (\textcolor{red}{$\uparrow$12.71\%}) & 90.40 (\textcolor{red}{$\uparrow$42.59\%}) \\
        GPT-4o               & 90.20 & 67.20 & 98.17 (\textcolor{red}{$\uparrow$08.84\%}) & 91.40 (\textcolor{red}{$\uparrow$36.01\%}) \\
        \bottomrule
    \end{tabular}
\label{tab_AdaCoder_accuracy}
\end{table*}

\begin{table*}
    \footnotesize
    \centering
    \caption{The pass@1 performance of selectd four multi-agent frameworks compared to the baseline when applied to six open-source models and four closed-source models on the MBPP benchmark.}
    \begin{tabular}{lccccc}
        \toprule
        \textbf{LLMs} & \textbf{Baseline} & \textbf{AgentCoder} & \textbf{MapCoder} & \textbf{INTERVENOR} & \textbf{Self-Collaboration} \\
        \midrule
        CodeLlama-Python-7B & 42.12 & 36.80 (\textcolor{cgreen}{$\downarrow$12.63\%}) & 55.00 (\textcolor{red}{$\uparrow$30.58\%}) & 47.00 (\textcolor{red}{$\uparrow$11.59\%}) & 35.20 (\textcolor{cgreen}{$\downarrow$16.43\%}) \\
        CodeLlama-Python-13B & 46.86 & 36.60 (\textcolor{cgreen}{$\downarrow$21.90\%}) & 61.60 (\textcolor{red}{$\uparrow$31.46\%}) & 53.00 (\textcolor{red}{$\uparrow$13.10\%}) & 40.40 (\textcolor{cgreen}{$\downarrow$13.79\%}) \\
        CodeLlama-Python-34B & 49.82 & 51.60 (\textcolor{red}{$\uparrow$03.57\%}) & 66.40 (\textcolor{red}{$\uparrow$33.28\%}) & 56.40 (\textcolor{red}{$\uparrow$13.21\%}) & 43.20 (\textcolor{cgreen}{$\downarrow$13.29\%}) \\
        DeepSeek-Coder-1.3B & 47.80 & 21.60 (\textcolor{cgreen}{$\downarrow$54.81\%}) & 37.40 (\textcolor{cgreen}{$\downarrow$21.76\%}) & 37.00 (\textcolor{cgreen}{$\downarrow$22.59\%}) & 38.60 (\textcolor{cgreen}{$\downarrow$19.25\%}) \\
        DeepSeek-Coder-6.7B & 58.60 & 60.20 (\textcolor{red}{$\uparrow$02.73\%}) & 44.60 (\textcolor{cgreen}{$\downarrow$23.89\%}) & 67.80 (\textcolor{red}{$\uparrow$15.70\%}) & 53.40 (\textcolor{cgreen}{$\downarrow$08.87\%}) \\
        DeepSeek-Coder-33B & 66.40 & 48.00 (\textcolor{cgreen}{$\downarrow$27.71\%}) & 60.40 (\textcolor{cgreen}{$\downarrow$09.04\%}) & 61.20 (\textcolor{cgreen}{$\downarrow$07.83\%}) & 53.20 (\textcolor{cgreen}{$\downarrow$19.88\%}) \\
        \bottomrule
    \end{tabular}
\label{tab_other_mbpp_accuracy}
\end{table*}

The results of AdaCoder with a maximum of $t = 5$ iterations on the HumanEval and MBPP datasets are presented in Table \ref{tab_AdaCoder_accuracy}. The performance of the other four frameworks on these datasets is shown in Table \ref{tab_overview_a} and Table \ref{tab_other_mbpp_accuracy}. The statistics indicate that AdaCoder achieves an average improvement of 54.58\% on HumanEval and 45.41\% on MBPP, totaling an average improvement of 50.00\%. In contrast, MapCoder, the most effective framework among the other four, only attains an average improvement of 50.43\% on HumanEval and 14.04\% on MBPP, resulting in a total average improvement of 32.24\%. These results demonstrate the superiority of AdaCoder.

% We applied AdaCoder to the six open-source models selected in RQ1 as foundation models, setting max iterations $t$ in algorithm \ref{algo_workflow} to be 5, and evaluated them on the HumanEval benchmark. The accuracy performance of AdaCoder is shown in Table \ref{tab_AdaCoder_open_accuracy}. As RQ1 demonstrated MapCoder's superior performance across all multi-agent framework, Table \ref{tab_AdaCoder_open_accuracy} only includes MapCoder as a representative of multi-agent frameworks for comparison. The results reveal that AdaCoder significantly enhances the code generation capabilities of open-source models, with improvement ranges from 40.57\% to 96.32\%. In contrast, the previously best-performing MapCoder showed improvements ranging from 04.72\% to 68.76\%, consistently underperforming AdaCoder across all six open-source models. On average, MapCoder improves code generation capability by 38.86\%, while AdaCoder achieves a 69.80\% improvement. Beyond overall performance enhancement, AdaCoder exhibits the following characteristics: 

% \begin{itemize}
%     \item [$\bullet$] Model architecture significantly influences AdaCoder's improvement effect: For CodeLlama-Python series models, AdaCoder's improvement ranges from 85.50\% to 96.32\%, averaging 91.93\%. For DeepSeek-Coder series models, the improvement spans from 40.57\% to 55.56\%, averaging 47.67\%, approximately half that of the CodeLlama-Python series. This indicates AdaCoder's preference for certain model architectures, though its minimum improvement remains substantial at 40.57\%.
%     \item [$\bullet$] AdaCoder's improvement effect negatively correlates with the foundation model's inherent performance: We plotted a scatter diagram using the baseline results of the six open-source LLMs as the x-axis and the improvement percentage after applying AdaCoder as the y-axis as shown in Figure \ref{fig_scatter_magnitude}. Linear regression analysis yielded the equation $y=-1.9292x+161.63$, with a goodness of fit $R^2=0.9196$, indicating a clear negative correlation between AdaCoder's improvement magnitude and the model's baseline results. We attribute this phenomenon to two factors: First, the Debug Specialist agent in AdaCoder, responsible for code error correction, employs rule-based debugging methods capable of fixing only simple issues. As model performance improves, the proportion of simple problems in generated code decreases, replaced by logical issues beyond the Debug Specialist's capability. Second, performance has an upper limit (100\%), naturally reducing the improvement potential for models with higher baseline accuracy.
% \end{itemize}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{image/scatter_magitude.pdf}
%     \caption{A scatter diagram using the baseline results of the six open-source LLMs as the x-axis and the improvement percentage after applying AdaCoder as the y-axis.}
%     \label{fig_scatter_magnitude}
% \end{figure}

In RQ2, we validated the ineffectiveness of Iteration Refinement by conducting repeated experiments with varying iteration counts $k$ across four selected multi-agent frameworks. Similarly, we performed repeated tests by adjusting the maximum iterations $t$ to 1, 2, 3, and 4, and plotted line graphs with $t$ values on the x-axis and test pass@1 on the y-axis, as shown in Figure \ref{fig_AdaCoder_open_t}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/AdaCoder_t_value.pdf}
    \caption{Line graphs with $t$ values as the x-axis and pass@1 as the y-axis.}
    \label{fig_AdaCoder_t_value}
\end{figure}

For open-source LLMs, increasing $t$ values significantly enhances the code generation capabilities. For instance, when AdaCoder uses CodeLlama-Python-34B as the foundation model, merely increasing $t$ from 1 to 2 improves pass@1 from 60.37\% to 72.56\%, an approximately 20\% increase. Even for the DeepSeek-Coder-6.7B model, which showed the smallest improvement, increasing $t$ from 1 to 5 still yielded a 13.72\% performance boost. Statistical analysis indicates that each unit increase in $t$ value results in an average 6.33\% improvement in model code generation capability. Furthermore, we compared the improvement magnitudes when increasing $t$ from 1 to 3 and from 3 to 5, finding them to be 20.44\% and 6.24\% respectively, with the latter significantly lower. This demonstrates a marginal effect in the improvement of code generation capabilities as $t$ values increase.

For closed-source LLMs, increasing $t$ values has a minimal impact on the code generation capabilities of closed-source LLMs. For instance, when AdaCoder uses GPT-4o as the foundation model, increasing $t$ from 1 to 5 only improves pass@1 from 94.51\% to 98.17\%, a mere 3.87\% increase. Among the four closed-source models, only GPT-4 showed a notable improvement when $t$ increased from 1 to 2: from 86.59\% to 93.29\%, a 7.74\% increase. Statistical analysis indicates that each unit increase in $t$ value results in an average improvement of only 1.69\% in model code generation capability. However, it is noteworthy that even with a single execution of the workflow shown in Figure \ref{fig_workflow}, these closed-source models perform exceptionally well, far surpassing baseline results. For example, GPT-4-turbo and GPT-4o achieved 93.29\% and 94.51\% pass@1 respectively with $t$ set to 1. Therefore, we posit that the limited improvement effect of AdaCoder on closed-source models is due to their inherently strong code generation capabilities. After just one round of the workflow shown in Figure \ref{fig_workflow}, their pass@1 is already very high, leaving limited room for improvement and resulting in the less pronounced enhancement effect of AdaCoder.


% \vspace{0.3cm}
% \begin{mdframed}[nobreak=true]
% \textbf{Answer:} Applying AdaCoder to open-source models significantly enhances code generation capabilities, with an average improvement of 69.80\% across six open-source LLMs, outperforming all four selected multi-agent frameworks. Increasing AdaCoder's $t$ value also significantly improves its code generation effect: for each unit increase in t, the code generation capability improves by an average of 6.33\%.
% \end{mdframed}


% \subsubsection{Accuracy Performance on Closed-source Models}

% \begin{table}
%     \footnotesize
%     \centering
%     \caption{The accuracy improvement of AdaCoder and four other multi-agent frameworks compared to the baseline when applied to the closed-source GPT series models.}
%     \begin{tabular}{lcccccc}
%         \hline
%         \textbf{LLMs} & \textbf{Baseline} & \textbf{AgentCoder} & \textbf{MapCoder} & \textbf{INTERVENOR} & \textbf{Self-Collaboration} & \textbf{AdaCoder} \\
%         \hline
%         GPT-3.5-turbo & 60.30 & 79.90 (\textcolor{red}{$\uparrow$32.50\%}) & 80.50 (\textcolor{red}{$\uparrow$33.50\%}) & 75.60 (\textcolor{red}{$\uparrow$25.37\%}) & 74.40 (\textcolor{red}{$\uparrow$23.38\%}) & 96.95 (\textcolor{red}{$\uparrow$60.78\%}) \\
%         GPT-4 & 67.00 & 96.30 (\textcolor{red}{$\uparrow$43.73\%}) & 93.90 (\textcolor{red}{$\uparrow$40.15\%}) & - & 90.20 (\textcolor{red}{$\uparrow$34.63\%}) & 96.95 (\textcolor{red}{$\uparrow$44.70\%}) \\
%         GPT-4-turbo & 87.10 & 89.60 (\textcolor{red}{$\uparrow$02.87\%}) & - & - & - & 98.17 (\textcolor{red}{$\uparrow$12.71\%}) \\
%         GPT-4o & 90.20 & - & - & - & - & 98.17 (\textcolor{red}{$\uparrow$08.84\%}) \\
%         \hline
%     \end{tabular}
% \label{tab_AdaCoder_close_accuracy}
% \end{table}

% We applied AdaCoder to GPT-3.5-turbo, GPT-4, GPT-4-turbo, and GPT-4o as foundation models, similarly setting $t$ to 5, and evaluated them on the HumanEval benchmark. The accuracy performance of AdaCoder is shown in Table \ref{tab_AdaCoder_close_accuracy}. The baseline performance for GPT-3.5-turbo is sourced from Wang et al.'s study \cite{wang2024intervenorpromptingcodingability}, while the baseline for the GPT-4 series is from OpenAI's GPT-4o introduction \cite{gpt4result}. The table also compares the performance of the four multi-agent frameworks selected in RQ1 on the GPT series models, with data sourced from their respective papers and unpublished data denoted by "-". Results indicate that AdaCoder significantly enhances the code generation capabilities of closed-source models, with improvements ranging from 8.84\% to 60.78\%. For GPT-3.5-turbo, MapCoder performed best among the other three frameworks with 80.50\% accuracy, still far behind AdaCoder's 96.95\%. For GPT-4, AgentCoder led with 96.30\%, approaching AdaCoder's 96.95\%. On GPT-4-turbo, only AgentCoder had experimental data at 89.60\%, lower than AdaCoder's 98.17\%. For OpenAI's recently released GPT-4o, the other frameworks lacked experimental data, while AdaCoder achieved 98.17\%, matching GPT-4-turbo. Consequently, AdaCoder achieved SOTA performance across all four closed-source models \cite{HumanEvalBenchmark}. 

% Similar to RQ3, we varied $t$ values to verify whether multiple executions of the workflow shown in Figure \ref{fig_workflow} could significantly enhance the code generation capabilities of closed-source models. We conducted tests with $t$ values of 1, 2, 3, and 4, recording the results. We plotted line graphs with $t$ values as the x-axis and test accuracy as the y-axis, illustrating AdaCoder's accuracy performance using the four selected closed-source LLMs as foundation models, as shown in Figure \ref{fig_AdaCoder_close_t}. 


% \vspace{0.3cm}
% \begin{mdframed}[nobreak=true]
% \textbf{Answer:} Applying AdaCoder to closed-source models similarly enhances code generation capabilities significantly, with an average improvement of 31.76\% across four closed-source LLMs, all achieving SOTA performance. However, increasing AdaCoder's $t$ value for closed-source models has a limited effect on improving code generation capability: for each unit increase in t, the code generation capability improves by an average of only 1.69\%.
% \end{mdframed}

\subsection{Resource Consumption Performance}\label{eva_resource}

% The statistics indicate that AdaCoder achieves an average improvement of 54.58\% on HumanEval and 45.41\% on MBPP, totaling an average improvement of 50\%. In contrast, MapCoder, the most effective framework among the other four, only attains an average improvement of 50.43\% on HumanEval and 14.04\% on MBPP, resulting in a total average improvement of 32.24\%. These results demonstrate the superiority of AdaCoder.

Although AdaCoder significantly enhances the performance of ten LLMs with varying parameter sizes, architectures, and performance levels, its practical value could be questioned if it consumes excessive computational resources and inference time similar to MapCoder. Therefore, we recorded the average token consumption and inference time required for AdaCoder to process a sample on the open-source models selected in RQ1. Given that the closed-source GPT series models operate on OpenAI's servers, measuring their inference time holds limited significance. Consequently, we only documented their token consumption, as illustrated in Table \ref{tab_AdaCoder_resource}. We also recorded the resource consumption data of the other four frameworks, as shown in Table \ref{tab_mbpp_resource}.

Analysis of the tabulated data reveals that in terms of token consumption, using AdaCoder results in an average increase of 2.00 times on HumanEval and 2.42 times on MBPP, totaling an average increase of 2.21 times. In contrast, the most effective framework among the other four, MapCoder, leads to an average increase of 23.02 times on HumanEval and 30.61 times on MBPP, resulting in a total average increase of 26.81 times, which is 12.13 times that of AdaCoder. Regarding inference time, using AdaCoder results in an average increase of 0.68 times on HumanEval and 1.34 times on MBPP, totaling an average increase of 1.01 times. While MapCoder leads to an average increase of 15.72 times on HumanEval and 16.35 times on MBPP, totaling an average increase of 16.04 times, which is 15.88 times that of AdaCoder. These results demonstrate AdaCoder's simplicity and efficiency.

% the application of MapCoder results in a substantial increase across all models, ranging from 19.69 to 26.20 times the baseline. CodeLlama-Python-7B exhibits the highest increase in token consumption, while CodeLlama-Python-34B shows the smallest increase, with an average increase of 23.02 times. In contrast, the application of AdaCoder leads to only modest increases in token consumption, ranging from 0.80 to 4.26 times the baseline. CodeLlama-Python-7B demonstrates the highest increase in token consumption under AdaCoder, while GPT-4o shows the smallest increase, with an average increase of only 2.00 times, approximately 1/12 of MapCoder's increase.

% Regarding inference time, the application of MapCoder similarly results in significant increases, ranging from 10.31 to 30.14 times the baseline. CodeLlama-Python-7B exhibits the highest increase in inference time, while CodeLlama-Python-34B shows the smallest increase, with an average increase of 15.72 times. Conversely, the application of AdaCoder leads to only minor increases in inference time, ranging from 0.27 to 0.91 times the baseline. CodeLlama-Python-34B demonstrates the highest increase in inference time under AdaCoder, while DeepSeek-Coder-1.3B shows the smallest increase, with an average increase of only 0.68 times, approximately 1/23 of MapCoder's increase.

\begin{table*}
\footnotesize
\centering
\caption{The resource consumption performance of AdaCoder on HumanEval and MBPP.}
\begin{subtable}[t]{\textwidth}
    \centering
    \caption{The average inference token consumption of AdaCoder on HumanEval and MBPP.}
    \begin{tabular}{l|c|c|c|c}
        \toprule
        \multirow{2}{*}{\textbf{LLMs}} & \multicolumn{2}{c|}{\textbf{Baseline}} & \multicolumn{2}{|c}{\textbf{AdaCoder}} \\ 
        \cline{2-5} & HumanEval & MBPP & HumanEval & MBPP \\
        \midrule
        CodeLlama-Python-7B  & 00.91K & 00.81K & 04.79K (\textcolor{red}{$\uparrow$04.26$\times$}) & 03.29K (\textcolor{red}{$\uparrow$03.07$\times$}) \\
        CodeLlama-Python-13B & 00.92K & 00.76K & 04.01K (\textcolor{red}{$\uparrow$03.36$\times$}) & 03.10K (\textcolor{red}{$\uparrow$03.09$\times$}) \\
        CodeLlama-Python-34B & 00.95K & 01.06K & 03.46K (\textcolor{red}{$\uparrow$02.64$\times$}) & 03.06K (\textcolor{red}{$\uparrow$01.89$\times$}) \\
        DeepSeek-Coder-1.3B  & 01.13K & 01.11K & 03.86K (\textcolor{red}{$\uparrow$02.42$\times$}) & 03.81K (\textcolor{red}{$\uparrow$02.42$\times$}) \\
        DeepSeek-Coder-6.7B  & 01.16K & 01.16K & 02.87K (\textcolor{red}{$\uparrow$01.47$\times$}) & 03.23K (\textcolor{red}{$\uparrow$01.78$\times$}) \\
        DeepSeek-Coder-33B   & 01.18K & 01.17K & 02.92K (\textcolor{red}{$\uparrow$01.47$\times$}) & 03.20K (\textcolor{red}{$\uparrow$01.75$\times$}) \\
        GPT-3.5-turbo        & 00.40K & 00.29K & 00.83K (\textcolor{red}{$\uparrow$01.07$\times$}) & 01.08K (\textcolor{red}{$\uparrow$02.72$\times$}) \\
        GPT-4                & 00.41K & 00.50K & 01.05K (\textcolor{red}{$\uparrow$01.56$\times$}) & 01.76K (\textcolor{red}{$\uparrow$02.54$\times$}) \\
        GPT-4-turbo          & 00.46K & 00.46K & 00.89K (\textcolor{red}{$\uparrow$00.93$\times$}) & 01.57K (\textcolor{red}{$\uparrow$02.42$\times$}) \\
        GPT-4o               & 00.37K & 00.41K & 00.66K (\textcolor{red}{$\uparrow$00.78$\times$}) & 01.43K (\textcolor{red}{$\uparrow$02.48$\times$}) \\
        \bottomrule
    \end{tabular}
\label{tab_AdaCoder_token}
\end{subtable}

\begin{subtable}[t]{\textwidth}
    \centering
    \vspace{0.5cm}
    \caption{The average inference time of AdaCoder on HumanEval and MBPP.}
    \begin{tabular}{l|c|c|c|c}
        \toprule
        \multirow{2}{*}{\textbf{LLMs}} & \multicolumn{2}{c|}{\textbf{Baseline}} & \multicolumn{2}{|c}{\textbf{AdaCoder}} \\ 
        \cmidrule{2-5} & HumanEval & MBPP & HumanEval & MBPP \\
        \midrule
        CodeLlama-Python-7B  & 27.33s & 15.12s & 48.61s (\textcolor{red}{$\uparrow$00.78$\times$}) & 32.88s (\textcolor{red}{$\uparrow$01.18$\times$}) \\
        CodeLlama-Python-13B & 41.42s & 21.85s & 70.24s (\textcolor{red}{$\uparrow$00.70$\times$}) & 69.80s (\textcolor{red}{$\uparrow$02.20$\times$}) \\
        CodeLlama-Python-34B & 76.49s & 70.53s & 145.9s (\textcolor{red}{$\uparrow$00.91$\times$}) & 144.7s (\textcolor{red}{$\uparrow$01.05$\times$}) \\
        DeepSeek-Coder-1.3B  & 22.52s & 12.06s & 28.55s (\textcolor{red}{$\uparrow$00.27$\times$}) & 30.38s (\textcolor{red}{$\uparrow$01.52$\times$}) \\
        DeepSeek-Coder-6.7B  & 20.65s & 20.90s & 35.55s (\textcolor{red}{$\uparrow$00.72$\times$}) & 43.29s (\textcolor{red}{$\uparrow$01.07$\times$}) \\
        DeepSeek-Coder-33B   & 88.27s & 86.59s & 149.2s (\textcolor{red}{$\uparrow$00.69$\times$}) & 176.4s (\textcolor{red}{$\uparrow$01.04$\times$}) \\
        \bottomrule
    \end{tabular}
\label{tab_AdaCoder_time}
\end{subtable}
\label{tab_AdaCoder_resource}
\end{table*}

\begin{table*}
\footnotesize
\centering
\caption{The resource consumption performance of AgentCoder, MapCoder, INTERVENOR and Self-Collaboration on MBPP.}
\begin{subtable}[t]{\textwidth}
    \centering
    \caption{The average inference token consumption of AgentCoder, MapCoder, INTERVENOR and Self-Collaboration on MBPP.}
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{LLMs} & \textbf{Baseline} & \textbf{AgentCoder} & \textbf{MapCoder} & \textbf{INTERVENOR} & \textbf{Self-Collaboration} \\
        \midrule
        CodeLlama-Python-7B & 00.81K & 12.18K (\textcolor{red}{$\uparrow$14.06$\times$}) & 32.46K (\textcolor{red}{$\uparrow$39.16$\times$})& 14.09K (\textcolor{red}{$\uparrow$16.43$\times$}) & 24.52K (\textcolor{red}{$\uparrow$29.33$\times$}) \\
        CodeLlama-Python-13B & 00.76K & 12.40K (\textcolor{red}{$\uparrow$15.37$\times$}) & 28.31K (\textcolor{red}{$\uparrow$36.37$\times$})& 12.06K (\textcolor{red}{$\uparrow$14.91$\times$}) & 18.88K (\textcolor{red}{$\uparrow$23.91$\times$}) \\
        CodeLlama-Python-34B & 01.06K & 10.48K (\textcolor{red}{$\uparrow$08.90$\times$}) & 24.74K (\textcolor{red}{$\uparrow$22.37$\times$})& 09.77K (\textcolor{red}{$\uparrow$08.22$\times$}) & 16.86K (\textcolor{red}{$\uparrow$14.92$\times$}) \\
        DeepSeek-Coder-1.3B & 01.11K & 14.49K (\textcolor{red}{$\uparrow$12.02$\times$}) & 33.06K (\textcolor{red}{$\uparrow$28.70$\times$})& 15.25K (\textcolor{red}{$\uparrow$12.70$\times$}) & 18.45K (\textcolor{red}{$\uparrow$15.58$\times$}) \\
        DeepSeek-Coder-6.7B & 01.16K & 08.79K (\textcolor{red}{$\uparrow$06.56$\times$}) & 37.78K (\textcolor{red}{$\uparrow$31.50$\times$})& 09.50K (\textcolor{red}{$\uparrow$07.18$\times$}) & 16.73K (\textcolor{red}{$\uparrow$13.39$\times$}) \\
        DeepSeek-Coder-33B & 01.17K & 10.29K (\textcolor{red}{$\uparrow$07.83$\times$}) & 30.95K (\textcolor{red}{$\uparrow$25.56$\times$})& 11.46K (\textcolor{red}{$\uparrow$08.84$\times$}) & 18.15K (\textcolor{red}{$\uparrow$14.57$\times$}) \\
        % GPT-3.5-turbo & 00.29K & - & - & - & - & 01.08K (\textcolor{red}{$\uparrow$00.00$\times$}) \\
        % GPT-4 & 00.50K & - & - & - & - & 01.76K (\textcolor{red}{$\uparrow$00.00$\times$}) \\
        % GPT-4-turbo & 00.46K & - & - & - & - & 01.57K (\textcolor{red}{$\uparrow$00.00$\times$}) \\
        % GPT-4o & 00.41K & - & - & - & - & 01.43K (\textcolor{red}{$\uparrow$00.00$\times$}) \\
        \bottomrule
    \end{tabular}
\label{tab_mbpp_tokens}
\end{subtable}
% \hfill
\begin{subtable}[t]{\textwidth}
    \vspace{0.5cm}
    \centering
    \caption{The average inference time of AgentCoder, MapCoder, INTERVENOR and Self-Collaboration on MBPP.}
    \begin{tabular}{lccccc}
        \toprule
        \textbf{LLMs} & \textbf{Baseline} & \textbf{AgentCoder} & \textbf{MapCoder} & \textbf{INTERVENOR} & \textbf{Self-Collaboration} \\
        \midrule
        CodeLlama-Python-7B  & 15.12s & 123.4s (\textcolor{red}{$\uparrow$07.16$\times$}) & 319.5s (\textcolor{red}{$\uparrow$20.14$\times$}) & 170.7s (\textcolor{red}{$\uparrow$10.29$\times$}) & 226.9s (\textcolor{red}{$\uparrow$14.01$\times$}) \\
        CodeLlama-Python-13B & 21.85s & 306.8s (\textcolor{red}{$\uparrow$13.04$\times$}) & 515.0s (\textcolor{red}{$\uparrow$22.57$\times$}) & 212.3s (\textcolor{red}{$\uparrow$08.72$\times$}) & 345.2s (\textcolor{red}{$\uparrow$14.80$\times$}) \\
        CodeLlama-Python-34B & 70.53s & 393.7s (\textcolor{red}{$\uparrow$04.58$\times$}) & 916.1s (\textcolor{red}{$\uparrow$11.99$\times$}) & 367.2s (\textcolor{red}{$\uparrow$04.21$\times$}) & 611.8s (\textcolor{red}{$\uparrow$07.67$\times$}) \\
        DeepSeek-Coder-1.3B  & 12.06s & 90.88s (\textcolor{red}{$\uparrow$06.54$\times$}) & 182.1s (\textcolor{red}{$\uparrow$14.10$\times$}) & 111.3s (\textcolor{red}{$\uparrow$08.23$\times$}) & 97.33s (\textcolor{red}{$\uparrow$07.07$\times$}) \\
        DeepSeek-Coder-6.7B  & 20.90s & 88.83s (\textcolor{red}{$\uparrow$03.25$\times$}) & 359.8s (\textcolor{red}{$\uparrow$16.22$\times$}) & 112.8s (\textcolor{red}{$\uparrow$04.40$\times$}) & 194.6s (\textcolor{red}{$\uparrow$08.31$\times$}) \\
        DeepSeek-Coder-33B   & 86.59s & 392.4s (\textcolor{red}{$\uparrow$03.53$\times$}) & 1217.2s (\textcolor{red}{$\uparrow$13.06$\times$}) & 541.5s (\textcolor{red}{$\uparrow$05.25$\times$}) & 706.0s (\textcolor{red}{$\uparrow$07.15$\times$}) \\
        \bottomrule
    \end{tabular}
\label{tab_mbpp_time}
\end{subtable}
\label{tab_mbpp_resource}
\end{table*}




% \begin{table}
% \footnotesize
% \caption{Changes in token consumption and inference time after applying AdaCoder to six open-source models and four closed-source models.}
% \centering
% \begin{subtable}[t]{\textwidth}
%     \centering
%     \caption{Changes in token consumption after applying AdaCoder to six open-source models and four closed-source models, "$\times$" represents multiple of increase.}
%     \begin{tabular}{lccccc}
%         \hline
%         \textbf{LLMs} & \textbf{Baseline} & \textbf{MapCoder} & \textbf{AdaCoder} \\
%         \hline
%         CodeLlama-Python-7B & 00.91K & 24.72K (\textcolor{red}{$\uparrow$26.20$\times$}) & 04.79K (\textcolor{red}{$\uparrow$04.26$\times$}) &  \\
%         CodeLlama-Python-13B & 00.92K & 21.79K (\textcolor{red}{$\uparrow$22.66$\times$}) & 04.01K (\textcolor{red}{$\uparrow$03.36$\times$}) & \\
%         CodeLlama-Python-34B & 00.95K & 19.72K (\textcolor{red}{$\uparrow$19.69$\times$}) & 03.46K (\textcolor{red}{$\uparrow$02.64$\times$}) & \\
%         DeepSeek-Coder-1.3B & 01.13K & 27.30K (\textcolor{red}{$\uparrow$23.20$\times$}) & 03.86K (\textcolor{red}{$\uparrow$02.42$\times$}) & \\
%         DeepSeek-Coder-6.7B & 01.16K & 29.92K (\textcolor{red}{$\uparrow$24.77$\times$}) & 02.87K (\textcolor{red}{$\uparrow$01.47$\times$}) & \\
%         DeepSeek-Coder-33B & 01.18K & 26.60K (\textcolor{red}{$\uparrow$21.58$\times$}) & 02.92K (\textcolor{red}{$\uparrow$01.47$\times$}) & \\
%         GPT-3.5-turbo & 00.40K & - & 00.83K (\textcolor{red}{$\uparrow$01.07$\times$}) \\
%         GPT-4 & 00.41K & - & 01.05K (\textcolor{red}{$\uparrow$01.57$\times$}) \\
%         GPT-4-turbo & 00.46K & - & 00.89K (\textcolor{red}{$\uparrow$00.93$\times$}) \\
%         GPT-4o & 00.37K & - & 00.66K (\textcolor{red}{$\uparrow$00.80$\times$}) \\
%         \hline
%     \end{tabular}
% \label{tab_AdaCoder_token}
% \end{subtable}

% \begin{subtable}[t]{\textwidth}
%     \centering
%     \vspace{0.5cm}
%     \caption{Changes in inference time after applying AdaCoder to six open-source models and four closed-source models, "$\times$" represents multiple of increase.}
%     \begin{tabular}{lccccc}
%         \hline
%         \textbf{LLMs} & \textbf{Baseline} & \textbf{MapCoder} & \textbf{AdaCoder} \\
%         \hline
%         CodeLlama-Python-7B & 27.33s & 850.97s (\textcolor{red}{$\uparrow$30.14$\times$}) & 48.61s (\textcolor{red}{$\uparrow$00.78$\times$})\\
%         CodeLlama-Python-13B & 41.42s & 781.62s (\textcolor{red}{$\uparrow$17.87$\times$}) & 70.24s (\textcolor{red}{$\uparrow$00.70$\times$})\\
%         CodeLlama-Python-34B & 76.49s & 865.02s (\textcolor{red}{$\uparrow$10.31$\times$}) & 145.91s (\textcolor{red}{$\uparrow$00.91$\times$})\\
%         DeepSeek-Coder-1.3B & 22.52s & 286.32s (\textcolor{red}{$\uparrow$11.71$\times$}) & 28.55s (\textcolor{red}{$\uparrow$00.27$\times$})\\
%         DeepSeek-Coder-6.7B & 20.65s & 292.74s (\textcolor{red}{$\uparrow$13.18$\times$}) & 35.55s (\textcolor{red}{$\uparrow$00.72$\times$})\\
%         DeepSeek-Coder-33B & 88.27s  & 1071.11s (\textcolor{red}{$\uparrow$11.13$\times$}) & 149.18s (\textcolor{red}{$\uparrow$00.69$\times$})\\
%         \hline
%     \end{tabular}
% \label{tab_AdaCoder_time}
% \end{subtable}
% \label{tab_AdaCoder_resource}
% \end{table}


\vspace{0.3cm}
\begin{mdframed}[nobreak=true]
\textbf{Answer to RQ3:} Applying AdaCoder to both open-source and closed-source LLMs can enhance their performance by an average of 50.00\%, surpassing existing multi-agent frameworks. Meanwhile, AdaCoder only increases the average token consumption and inference time by 2.21 times and 1.01 times, respectively, which are approximately one twelfth and one sixteenth of those required by the exsiting most effective framework, MapCoder.
\end{mdframed}
